A Neural Score Follower for Computer Accompaniment of Polyphonic Musical Instruments

Real-time computer-based accompaniment for human musical performances entails three critical tasks: identifying what the performer is playing, locating their position within the score, and synchronously playing the accompanying parts. Among these, the second task (score following) has been addressed through methods such as dynamic programming on string sequences, Hidden Markov Models (HMMs), and Online Time Warping (OLTW). Yet, the remarkably successful techniques of Deep Learning (DL) have not been directly applied to this problem. Therefore, we introduce HeurMiT, a novel DL-based score-following framework, utilizing a neural architecture designed to learn compressed latent representations that enables precise performer tracking despite deviations from the score. Parallelly, we implement a real-time MIDI data augmentation toolkit, aimed at enhancing the robustness of these learned representations. Additionally, we integrate the overall system with simple heuristic rules to create a comprehensive framework that can interface seamlessly with existing transcription and accompaniment technologies. However, thorough experimentation reveals that despite its impressive computational efficiency, HeurMiT's underlying limitations prevent it from being practical in real-world score following scenarios. Consequently, we present our work as an introductory exploration into the world of DL-based score followers, while highlighting some promising avenues to encourage future research towards robust, state-of-the-art neural score following systems.

==> fontsets/mitthesis-defaultfonts.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-defaultfonts.tex}[2023/09/12 v1.03 Load Computer/Latin Modern text and math fonts]

%% Default fonts
%
\ifpdftex
	\typeout{^^JLoading Computer Modern text and math fonts (default for pdftex).^^J}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\typeout{^^JLoading Latin Modern text and math fonts (default for unicode engines).^^J}
	%
	\RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
	% suppress tiresome warnings about lack of integration between mathtools and unicode-math.
	% Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-fira-newtxsf.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-fira-newtxsf.tex}[2023/09/12 v1.04 Load Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font]

%% Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font
%
\ifpdftex
    \typeout{^^JLoading Fira sans text font with newtx sans serif math font and Inconsolata typewriter^^J}
    \RequirePackage[sfdefault,scaled=0.90]{FiraSans} % sans serif text package %,scaled=.85
    \RequirePackage[T1]{fontenc}
    \RequirePackage[varqu,varl,scaled=1.05]{zi4} % inconsolata font for typewriter
    \RequirePackage[scaled=1.05]{newtxsf} % sans serif math
    \RequirePackage{bm}
\else
    \ClassWarning{mitnewthesis}{The fira-newtxsf font set requires pdflatex. Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-heros-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-heros-stix2.tex}[2023/09/12 v1.02 Load TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font]

%% TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font
%
% These fonts are available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The heros-stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\typeout{^^JTeX Gyre Heros (sans serif) text font with STIX2 math font and Inconsolata monospaced font.^^J}
	%
	\RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
	% suppress tiresome warnings about lack of integration between mathtools and unicode-math
	% unicode-math loads the fontspec package

	\setmainfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
		UprightFont = *-regular,
		ItalicFont = *-italic,
		BoldFont = *-bold,
		BoldItalicFont = *-bolditalic,
		Numbers = Lining,
		Scale=0.91,
	]
	\setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
		UprightFont = *-regular,
		ItalicFont = *-italic,
		BoldFont = *-bold,
		BoldItalicFont = *-bolditalic,
		Numbers = Lining,
		Scale=0.91,
	]
	\setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package and is in CTAN https://ctan.org/tex-archive/fonts/inconsolata
		Scale=1.05,
		Extension = .otf,
		UprightFont = *-Regular,
		ItalicFont = *-Regular,% has no italic face
		BoldFont = *-Bold,
		BoldItalicFont = *-Bold,% has no bold italic face
		RawFeature = {+ss01,+ss02,+ss03},
	]
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed %% https://github.com/stipub/stixfonts
		Scale=MatchUppercase,
		Extension = .otf,
		BoldFont = *,% STIX Two Math has no bold face
		%       Color=NavyBlue, 
		RawFeature = {+ss01, -ss02, -ss08},
	]
	% ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
	%    
	\setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Heros bold, https://github.com/stipub/stixfonts
	\setmathfontface\mathit{STIXTwoText-Italic.otf}[]
	\setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX Two
	%         
	\newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-libertine.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-libertine.tex}[2023/09/12 v1.02 Load Libertine and related fonts]

%% Linux Libertine (serif) text font with newtxmath[libertine] (pdftex) or Libertinus (unicode) math font
%
%  These fonts are available here https://ctan.org/tex-archive/fonts/libertine/opentype 
%						 and here https://github.com/alerque/libertinus
% install these as system fonts on your computer
%
\ifpdftex
	\typeout{^^JLoading newtx-libertine text and math fonts with Insolata typewriter font^^J}
	\RequirePackage[lining,semibold]{libertine}
	\RequirePackage[T1]{fontenc}
	\RequirePackage[varqu,varl]{inconsolata}% typewriter
	%    \usepackage{amsthm}% must be loaded before newtxmath
	\RequirePackage[libertine,vvarbb]{newtxmath}
	\RequirePackage{bm}% load after all math to give access to bold math
\else
	\typeout{^^JLoading Linux Libertine (serif) text font with Libertinus math font^^J}
	%
	\RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
	% suppress tiresome warnings about lack of integration between mathtools and unicode-math
	% unicode math loads the fontspec package
	%
	\setmainfont{LinLibertine}[% Linux Libertine O  
		Extension = .otf,
		UprightFont = *_R,
		ItalicFont = *_RI,
		BoldFont = *_RZ, % Libertine O Semibold
		BoldItalicFont = *_RZI, % Libertine O Semibold Italic
		%	Ligatures=Rare,% TeX
		%	Numbers=OldStyle,%
		RawFeature={+ss05},% +ss02 would change J, K, R; +ss05 changes W	
	]
	\setmonofont{LinLibertine}[% Linux Libertine Mono O
		Scale=0.9,
		Extension = .otf,
		UprightFont = *_M,
		ItalicFont = *_MO,% oblique
		BoldFont = *_MB,
		BoldItalicFont = *_MBO,% oblique
	]
	\setsansfont{LinBiolinum}[% Linux Biolinum O
		Extension = .otf,
		UprightFont = *_R,
		ItalicFont = *_RI,
		BoldFont = *_RB,
		BoldItalicFont = *_RBO,% oblique
		Scale=MatchUppercase]
	%    	
	%% a Libertine-style math font
	\setmathfont{libertinusmath-regular}[%
		Extension = .otf,
		Scale=MatchUppercase,
		BoldFont = *,% This font lacks a bold version
		RawFeature={+ss08},% +ss08 gives slanted integrals (no other features) 	
	]
	\newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2}   
\fi


==> fontsets/mitthesis-lucida.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-lucida.tex}[2023/09/12 v1.02 Load Lucida fonts]

%% Lucida Bright and Lucida Bright Math fonts (available from the TeX Users Group)

\typeout{^^JLucida Bright and Lucida Bright Math fonts^^J}

\ifpdftex
  \RequirePackage[LY1]{fontenc}
  \RequirePackage[expert,vargreek,altbullet,seriftt]{lucidabr}   % switch text and math fonts
  \RequirePackage{bm}
\else
  \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
  % suppress tiresome warnings about lack of integration between mathtools and unicode-math
  % unicode-math loads the fontspec package

  % FEATURE 	DESCRIPTION 											DEFAULT
  % dlig 		discretionary ligatures (f-ligatures in typewriter fnt) off
  % liga 		standard ligatures (f-ligatures, not monospaced fonts) 	on
  % onum 		old style numbers (Lucida Bright only)					off
  % smcp 		small caps 	(Lucida Bright, upright only)				off
  % zero 		slashed zero (sans and monospaced fonts)				off
  % locl 		script/language specific (localized) forms 				on
  %
  % FEATURE 	FONT 						DESCRIPTION
  % ss01 		Lucida Sans & Typewriter 	use dotted zero: 𝟶 vs. default 0.
  % ss01 		use Lucida-standard shapes:
  % 			Lucida Grande Mono 			ØOQ vs. default 0OQ;
  % 			Lucida Console 				ØOQ vs. default 0OQ.

  \setmainfont{LucidaBrightOT}[% main rm
    Ligatures=TeX,
    Extension=.otf,
    UprightFont=*,
    ItalicFont=*-Italic,
    BoldFont=*-Demi,
    BoldItalicFont=*-DemiItalic,
    BoldItalicFeatures={Color=Purple4},
    %     UprightFeatures={Color=Salmon3},
    Scale=0.92,
    %	  Numbers ={OldStyle}, 
  ]
  %
  \setsansfont{LucidaSansOT}[% main sans
    Ligatures=TeX,
    Extension=.otf,
    UprightFont=*,
    ItalicFont=*-Italic,
    BoldFont=*-Demi,
    BoldItalicFont=*-DemiItalic,
    Scale=MatchUppercase,
  ]
  %
  \setmonofont{LucidaSansTypewriterOT}[% main typewriter
    Ligatures=TeX,
    Extension=.otf,
    UprightFont=*,
    ItalicFont=*-Oblique,
    BoldFont=*-Bold,
    BoldItalicFont=*-BoldOblique,
    Scale=MatchUppercase,
  ]

  %% MATH FONTS
  %
  % ss01 	alternate Latin lower case math italic identical to text italic. This option is not recommended as Greek 𝜈 (nu) and Latin 𝑣 (vee) become too similar
  % ss02 	smaller arrows (original Type 1 size): ⇑ vs. default ⇑.
  % ss03 	attempt to imitate Type 1 fonts
  % ss04 	calligraphic alternative (similar to the Type 1 design) to the math script alphabet
  % ss05 	use a slashed-zero style for the empty set character (U+2205): Ø vs. default ∅
  % ss08 	emphasize right and bottom edges of the d’Alembertian operator (U+29E0, \laplac), to follow the design of the Laplace operator (U+2206, \increment, Δ); the default design emphasizes the left and upper edges. Also available in the bold math font.
  %
  \setmathfont{LucidaBrightMathOT}[% main math
    Scale=MatchUppercase,
    Extension=.otf,
    BoldFont=LucidaBrightMathOT-Demi.otf,
    %    	  BoldFeatures={Color=Chartreuse4},
    RawFeature ={+ss04,+ss08}, %
  ]

  %% LucidaMath-OT contains a *serif* typerwriter font. If you prefer a sans serif typerwriter font, you can use the following two settings. 
  % 
  %    \setmathfont{LucidaSansTypewriterOT}[% <== NB: setting a text font where math font should go.
  %    	  Scale=MatchUppercase,
  %          range=tt,
  %    	  Color=NavyBlue,
  %          Extension=.otf,
  %          script-features = {},     
  %          sscript-features = {},     
  %    	  BoldFont=LucidaSansTypewriterOT-Bold.otf,
  %    	  BoldFeatures={Color=Salmon3},
  %    ]
  %    %
  %    \setmathfontface\mathtt{LucidaSansTypewriterOT-Bold}[% bold upright typewriter font in boldmath.
  %    	  version=bold,
  %    	  Scale=MatchUppercase,
  %          Extension=.otf,    
  %    ]
  %
  \setmathfont{LucidaBrightMathOT}[%
    range={scr},% to make scr differ from cal
    RawFeature={-ss04},
    Scale=MatchUppercase,
    Extension=.otf,
    BoldFont=LucidaBrightMathOT-Demi.otf,% could be overridden by bold separate version
  ]
  \setmathfont{LucidaBrightMathOT}[% -Demi .. sufficient this way, since bold set above.
    range={bfscr},% need to call \symbfscr manually - bug in unicode-math version & range interaction
    RawFeature={-ss04},
    Scale=MatchUppercase,
    Extension=.otf,
    BoldFont=LucidaBrightMathOT-Demi.otf,
  ]
  %% Fix unicode-math operator font not set up for bold face (default \mathrm). See https://github.com/wspr/unicode-math/issues/468
  \setoperatorfont\normalfont
  %
  % note \mathbfit = \symbfit

  % The specialized one-off Lucida fonts:
  \newfontface\LucidaBlackletter{LucidaBlackletterOT}[%
    Scale=0.95,% <== NB
    Extension=.otf,
  ]
  \newfontface\LucidaCalligraphy{LucidaCalligraphyOT}[%
    Scale=MatchUppercase,
    Extension=.otf,
  ]
  \newfontface\LucidaHandwriting{LucidaHandwritingOT}[%
    Scale=MatchUppercase,
    Extension=.otf,
  ]
  % GrandeMono and Console fonts:
  \newfontface\LucidaGrandeMonoDK{LucidaGrandeMonoDK}[%	
    Scale=MatchUppercase,
    Extension=.otf,
    UprightFont=*,
    ItalicFont=*-Italic,
    BoldFont=*-Bold,
    BoldItalicFont=*-BoldItalic,
  ]
  \newfontface\LucidaConsole{LucidaConsoleDK}[%
    Scale=MatchLowercase,% <=== NB
    Extension=.otf,
    UprightFont=*,
    ItalicFont=*-Italic,
    BoldFont=*-Bold,
    BoldItalicFont=*-BoldItalic,
  ]
\fi


==> fontsets/mitthesis-newtx-sans-text.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx-sans-text.tex}[2023/09/12 v1.02 Load newtx sans-serif text and regular math fonts]

%% newtx package with sans-serif text (Helvetica-like text with Times-like math)
%
\ifpdftex
    \RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91,defaultsups]{newtx}% upint for upright integrals
    \renewcommand{\familydefault}{\sfdefault}% use sans for main text
    %   these two commands enable hyphenation of the typewriter font - https://tex.stackexchange.com/a/204421/119566
    %    \input{t1ntxtt.fd}
    %    \DeclareFontFamily{\encodingdefault}{\ttdefault}{\hyphenchar\font=`\-} % 
    \RequirePackage{bm}% bold math
\else
    \ClassWarning{mitnewthesis}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi



==> fontsets/mitthesis-newtx.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx.tex}[2023/09/12 v1.03 Load newtx text and math fonts]

\ifpdftex
    \typeout{^^JLoading newtx fonts with inconsolata typewriter^^J}
    \RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91]{newtx}% stix2, upint
    \RequirePackage[varl,varqu,hyphenate,mono]{inconsolata}% sans typewriter font; mono = fixed word spacing, hyphenate = allow hyphenation 
    \RequirePackage{bm}
    \let\textsuperscript\textsu% newtx changes the default superiors font; this is needed to get commas aligned in sequential footnotes
\else
    \ClassWarning{mitnewthesis}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi



==> fontsets/mitthesis-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-stix2.tex}[2023/09/12 v1.03 Load STIX Two text and math fonts]

%% STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font
%
% These fonts are available at: 
%				https://github.com/stipub/stixfonts 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\typeout{^^JLoading STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font.^^J}
	%
	\RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
	% suppress tiresome warnings about lack of integration between mathtools and unicode-math
	% unicode-math loads the fontspec package
	%
	\setmainfont{STIXTwoText}[% Presumes these are system fonts! 
		Extension = .otf,
		UprightFont = *-Regular,
		ItalicFont = *-Italic,
		BoldFont = *-Bold,
		BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
	]
	\setsansfont{texgyreheros}[% Presumes these are system fonts! 
		WordSpace = {1,1.4,1},
		Extension = .otf,
		UprightFont = *-regular,
		ItalicFont = *-italic,
		BoldFont = *-bold,
		BoldItalicFont = *-bolditalic,
		Numbers = Lining,
		Scale=0.91,% 
	]
	\setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package (it's in TeX Live)
		Scale=1.05,%
		Extension = .otf,
		UprightFont = *-Regular,
		ItalicFont = *-Regular,% has no italic face
		BoldFont = *-Bold,
		BoldItalicFont = *-Bold,% has no bold italic face
		RawFeature = {+ss01,+ss02,+ss03},
	]
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed
		Scale=MatchUppercase,
		Extension = .otf,
		BoldFont = *,% STIX Two Math has no bold face
		%       Color=NavyBlue, 
		RawFeature = {+ss01, -ss02, -ss08},
	]
	% ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
	%
	\newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-termes-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-termes-stix2.tex}[2023/09/12 v1.03 Load TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font]

%% TeX Gyre Termes text font and Heros sans serif font with STIX2 math font and Inconsolata monospaced font
%
% These fonts are available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The termes-stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\typeout{^^JLoading TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font.^^J}
	%
	\RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
	% suppress tiresome warnings about lack of integration between mathtools and unicode-math
	% unicode-math loads the fontspec package
	%
	\setmainfont{TeXGyreTermesX}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},%% This stretch matches newtxtext a little better. 1.4
		Extension = .otf,
		UprightFont = *-Regular,
		ItalicFont = *-Italic,
		BoldFont = *-Bold,
		BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
	\setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
		UprightFont = *-regular,
		ItalicFont = *-italic,
		BoldFont = *-bold,
		BoldItalicFont = *-bolditalic,
		Numbers = Lining,
		Scale=0.91,% same as for newtx; former value 0.9 too small 2022/01/15
	]
	\setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package (it's in TeX Live)
		Scale=1.05,% rescaled from 1, 22/03/10
		Extension = .otf,
		UprightFont = *-Regular,
		ItalicFont = *-Regular,% has no italic face
		BoldFont = *-Bold,
		BoldItalicFont = *-Bold,% has no bold italic face
		RawFeature = {+ss01,+ss02,+ss03},
	]
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed %% https://github.com/stipub/stixfonts
		Scale=MatchUppercase,
		Extension = .otf,
		BoldFont = *,% STIX Two Math has no bold face
		%       Color=NavyBlue, 
		RawFeature = {+ss01, -ss02, -ss08},
	]
	% ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
	%
	\setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Termes bold, https://github.com/stipub/stixfonts
	\setmathfontface\mathit{STIXTwoText-Italic.otf}[]
	\setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX, not Termes
	%      
	\newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-termes.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-termes.tex}[2023/09/12 v1.03 Load TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font]

%% TeX Gyre Termes (Times-like) text font with Termes math font and Heros sans serif font and Cursor monospaced font
%
% These fonts are available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
% install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The termes fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\typeout{^^JLoading TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font^^J}
	\RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
	% suppress tiresome warnings about lack of integration between mathtools and unicode-math
	% unicode-math loads the fontspec package
	%
	\setmainfont{TeXGyreTermesX}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
		UprightFont = *-Regular,
		ItalicFont = *-Italic,
		BoldFont = *-Bold,
		BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
	\setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
		UprightFont = *-regular,
		ItalicFont = *-italic,
		BoldFont = *-bold,
		BoldItalicFont = *-bolditalic,
		Numbers = Lining,
		Scale=0.91,% same as for newtx; former value 0.9 too small 2022/01/15
	]
	\setmonofont{texgyrecursor}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		Scale=0.97,
		Extension = .otf,
		UprightFont = *-Regular,
		ItalicFont = *-Italic,
		BoldFont = *-Bold,
		BoldItalicFont = *-BoldItalic,
		%		BoldFeatures = { Color = VioletRed3 },
	]
	\setmathfont{texgyretermes-math}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		Scale=MatchUppercase,
		Extension = .otf,
		BoldFont = *, % termes-math does not have a bold version
		%       Color=Red3, 
	]
	%   
	\newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2}
\fi


==> mydesign.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mydesign.tex}[2023/10/11 v1.03 Typographic design options for thesis]

%%%%%%%%%%  Color support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Color package: xcolor. 
%% Change this if you prefer something else

\usepackage[hyperref,dvipsnames,svgnames,x11names]{xcolor}

%% can add option [table] to xcolor to use color in tables (see xcolor documentation)


%%%%%%%%%%  Hyperlink and line number colors  %%%%%%%%%%%%%%

\AtBeginDocument{
	% Using color names from xcolor package
	\hypersetup{
		linkcolor=Blue3,
		citecolor=Blue3,
		urlcolor=violet,
		filecolor=red,
		%	anchorcolor=yellow,%  not all pdf viewers recognize this field (although Firefox does): hyperref issues a warning
		%	colorscheme=phelype,% overrides link, cite, url, file colors with a preset scheme, through \DocumentMetadata
	}
	%
	\ifmit@lineno
		\renewcommand{\linenumberfont}{\sffamily\mdseries\tiny\color{violet}}% line numbers will be sans-serif, medium weight, tiny, and violet
	\fi
}

%%%%%%%%%  Caption support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% see documentation for details of how to customize captions

\RequirePackage{caption}
\RequirePackage{subcaption}


%%%%%%%%%  Customize list environments  %%%%%%%%%%%%%%%%%%%%
% 
% see documentation for details of how to customize lists

%\RequirePackage{enumitem}


%%%%%%%%%  Customize titles and section headings  %%%%%%%%%%
% 
% see documentation for details of how to customize headings

\RequirePackage{titlesec}

% these titlesec commands just automate the bold math in some headings (rest follows default styles)
\titleformat{\section}{\mathversion{bold}\normalfont\Large\bfseries}{\thesection }{1em}{}
\titleformat{\subsection}{\mathversion{bold}\normalfont\large\bfseries}{\thesubsection}{1em}{}
\titleformat{\subsubsection}{\mathversion{bold}\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{}

% ==> NOT every font includes a bold math version, so you may need to use other math macros in the headings to get bold math <==


%%%%%%%%%  Change page margins  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% The default thesis margin is 1 inch all around. You may want different margins (e.g., to add a gutter for binding),
% in which case you can use the \newgeometry command from the geometry package.  Refer to the package documentation
% for details.
%
% mitthesis defaults: [top=1in,bottom=1in,left=1in,right=1in,marginparwidth=50pt,headsep=12pt,footskip=0.5in]
%
% The following tells the geometry package to use a two-sided layout with a 1 cm binding offset on the inside 
% 	and 1 inch margins all around, reducing textwidth slightly (by 0.7 cm). See geometry documentation, Section 8.2.
%
%\newgeometry{twoside, bindingoffset=1cm,margin=1in,marginparwidth=50pt,headsep=12pt,footskip=0.5in}

